When Should we Expect Non-Decreasing Returns from Data in Prediction Tasks?

This article studies the change in the prediction accuracy of a response variable when the number of predictors increases, and all variables follow a multivariate normal distribution. Assuming that the correlations between variables are independently drawn, I show that adding variables leads to globally increasing returns to scale when the mean of the correlation distribution is zero. The speed of learning depends positively on the variance of the correlation distribution. I use simulations to study the more complex case of correlation distributions with a non-zero mean and find a pattern of decreasing returns followed by increasing returns to scale - as long as the variance of correlations is not degenerate, in which case globally decreasing returns emerge. I train a collaborative filtering algorithm using the MovieLens 1M dataset to analyze returns from adding variables in a more realistic setting and find globally increasing returns to scale across $2,000$ variables. The results suggest significant scale advantages from additional variables in prediction tasks.

==> subtex/lit.tex <==
%!TEX root = ../data_learning.tex

Our work is most directly related to the empirical literature investigating how additional data influences prediction accuracy. \cite{chiou2017search} exploit changes in the retention policy of search engine logs to analyze the effect of historical data on search result accuracy. \cite{klein2022important} conduct an experiment to assess the effect of additional data for the quality of search results and find evidence consistent with decreasing returns to scale.  \cite{peukert2024editor} find decreasing returns in prediction accuracy from prior user visits in the context of news recommendation. 

The aforementioned studies do not emphasize the multi-dimensional nature of data. \cite{bajari2019impact} are among the first to analyze potential interaction effects of different data dimensions in the context of Amazon's sales forecasts system. They find evidence for decreasing returns to scale both for the number of periods a product has been available for sale, and for the number of products within a product category. Their setting differs from ours as it assumes a fixed set of observed and unobserved explanatory variables for the sales forecast of a given product. 

\cite{lee2021recommender} study the value of user data for the prediction accuracy of recommender systems. Their article contains an empirical section in which they study the effect of adding variables on prediction accuracy. The authors consider a maximum of nine conditioning variables, a number our simulations suggest might be far below the threshold necessary to uncover increasing returns to scale. \cite{ullrich2024returns} analyze returns to data in the context of web tracking and find evidence for decreasing returns to scale in the number of users and in the number of tracked websites. While the number of tracked websites affects how many variables are available about users, both are not the same because not all users visit all of the tracked websites. This is a departure from out setting which assumes the same number of variables is observed across a large number of observations.\footnote{Interestingly, however, \cite{ullrich2024returns} note that decreasing returns to scale are more pronounced for the number of observations than for the number of variables, an observation that aligns with our findings.}   
 
Concluding that ``personalization based on short-term history [...] is [...] less valuable than long-term [...] personalization''  in the context of search engine recommendation, \cite{yoganarasimhan2020search} finds evidence broadly consistent with non-decreasing returns to scale from longer user histories, which is a proxy for the number of variables observed about users. In a similar context, \cite{schaefer2023complementarities} find increasing returns to scale for search result accuracy when a search engine query benefits from a longer average user history. The only article we are aware of which also focuses the research question on the effect of adding variables is \cite{hocuk2022economies} who use health record data to predict health outcomes for varying $K$ while holding  $N$ fixed. In their empirical setting, which is very similar to ours, the authors find evidence consistent with increasing returns to scale. 
 
 %on search result accuracy and finds evidence in line with non-decreasing returns to scale, concluding that ``personalization based on short-term history or within-session behavior is shown to be less valuable than long-term or across-session personalization.'' 

==> subtex/simulation.tex <==
%!TEX root = ../data_learning.tex

\subsection{The Multivariate Normal Distribution}

We study learning from variables by assuming that the K-dimensional variable vector $\mathbf{x} = (x_1,...,x_K)$ follows a multivariate normal distribution with mean vector $\bm{\mu}$ and covariance matrix $\bm{\Sigma}$. Using an arbitrary subset of variables $\mathbf{x_k} \in \mathbf{x}$ as the conditioning set for one other arbitrary variable, $y$, in the complementary set ($y \in \mathbf{x} \backslash \mathbf{x_k}$), the conditional variance of $y$ given $\mathbf{x_k}$ is given by: 

\begin{equation}\label{eq:multnorm}
	\sigma_{y|\mathbf{x_k}} = \sigma_y - \Sigma_{y,\mathbf{x_k}}(\Sigma_{\mathbf{x_k},\mathbf{x_k}})^{-1}\Sigma_{y,\mathbf{x_k}}.
\end{equation}

\noindent In \cref{eq:multnorm} $\sigma_y$ denotes the unconditional variance of variable $y$, $\Sigma_{y,\mathbf{x_k}}$ denotes the vector collecting the covariances between $y$ and each element of $\mathbf{x_k}$, and $\Sigma_{\mathbf{x_k},\mathbf{x_k}}$ denotes the conformable covariance matrix of the conditioning variables $\mathbf{x_k}$. Throughout our analysis, we normalize the mean vector to zero and the unconditional variances to one. As a result, the covariances become correlations. 

The conditional variance in \cref{eq:multnorm} corresponds to the residual variance of a linear regression model where the variable $y$ is predicted based on the variable vector $\mathbf{x_k}$.  As a result, the conditional variance in \cref{eq:multnorm} allows to study the effect of adding variables for the prediction accuracy, as measured by the variance of the prediction error, in the canonical linear regression model if the data generating process follows the multivariate normal distribution. 

\cref{eq:multnorm} has properties that make it suitable as an abstraction for prediction models more broadly. First, higher correlations between the predictors and the dependent variable will, all else equal, reduce the conditional variance. This captures the notion that variables with a more precise signal about the dependent variable will increase the prediction accuracy. Second, a higher correlation between the predictors will, all else equal, increase the conditional variance. This captures the notion that adding variables with similar information will generally not contribute to improve the prediction accuracy significantly.\footnote{In the context of linear regression, this manifests as the multicolinearity problem, which leads to high variances of the coefficients.}       

\subsection{Simulation Details}

\cref{alg:simulation} provides the details of our simulation approach. For a variable vector of dimension $K$ and a distribution $F(\cdot)$ of the correlation coefficients, we simulate $N$ learning trajectories. For each learning trajectory, we randomly select one prediction target $y$ from the variable vector $\mathbf{x}$, and draw the off-diagonal elements of the correlation matrix from the assumed correlation distribution $F(\cdot)$. 

We incrementally increase the number of predictive variables from $k=1$ to $k=K-1$ by randomly adding one new variable in every iteration of the inner loop. After implementing \cref{alg:simulation}, we obtain $N$ learning trajectories of length $K-1$. We are interested in the average learning trajectory obtained from averaging $\sigma_{y|\mathbf{x_k}}$ across the $N$ simulations for each value of $k$ in $1$ to $K-1$. 

\begin{algorithm}
	\caption{Simulation Algorithm}\label{alg:simulation}
	\begin{algorithmic}[1]
		\State \textbf{set} $K$ and $F(\cdot)$
		\For{$i$ in $1$ to $N$}
		\State \textbf{draw} $K(K-1)/2$ correlation coefficients
		\Statex independently from $F(\cdot)$
		\State \textbf{select} $y$ randomly from $\mathbf{x}$
		\State \textbf{set} $x_k = \emptyset$
		\For{$k$ in $1$ to $K-1$}
		\State \textbf{select} $x_k$ randomly from $\mathbf{x}\backslash(y \cup \mathbf{x_k})$
		\State \textbf{update} $\mathbf{x_k} \gets x_k$ 
		\State \textbf{compute} $\sigma_{y|\mathbf{x_k}}$ using \cref{eq:multnorm}
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

In the simulations presented in the main body of this article (\cref{sec:results}), we set $K=101$ and increase the number of conditioning variables from $k=1$ to $k=100$. We selected parametrizations of the correlation distributions to illustrate the main properties of learning from additional variables when $K=101$. In \cref{app:long_sims}, we show results for $K=501$ to demonstrate that, by decreasing the variance of the correlation distribution, it is easy to generate learning curves for which learning takes longer without affecting the main insights generated from our simulations based on $K=101$.

\subsection{Nearest Correlation Matrix Correction}  

\subsection{Discussion of Simulation Approach}

\subsubsection*{Interpretation}

\cref{alg:simulation} can be understood as mimicking the scenario in which a firm accumulates variables in a random order and seeks to predict another, yet unobserved, variable. An example of such a scenario is the recommendation problem in which a firm seeks to predict the taste of a consumer for a collection of items $K$. As consumers interact with the recommendation system, the firm gathers new additional variables about the consumer. For example, whether she liked past recommendations, or how long she interacted with past recommendations. 

The firm is not in full control over the sequence in which variables accumulate, as this is partly determined by the prompts of the consumer, which are driven by her idiosyncratic tastes.  Whenever the consumer prompts the recommendation engine about a new item, the firm provides a recommendation using a prediction model estimated based on the observed behavior of other users, who already interacted with the item. The quality of the prediction for the user will be determined by the precision of the signal that past variables provide for the new item, estimated by the model which uses data about the other users.   

Thus, our approach may be viewed as shedding light on how the prediction quality for a single user changes, when she joins a service with a large user base who have already provided the firm with ample observation to estimate the relationship between variables.  Alternatively, our simulations can be thought of as mimicking the scenario in which a firm with many users (i.e., observations) acquires new variables for a large number of its users simultaneously. This may, for example be the case, when a firm buys data about its users (merger), or if a firm shows a new item to many users simultaneously (when running an ad campaign). In this scenario, the firm acquires a new signal about many of its users simultaneously which it can use to predict future variables. In this case, acquiring a new variable changes the prediction quality for many users simultaneously.     

In our baseline analysis, we use Beta Distributions with various parametrizations to draw the correlations from. This is primarily motivated by the fact that the Beta Distribution is bounded between $0$ and $1$ and therefore presents itself as a natural first choice when drawing correlations. We distinguish between distributions centered around zero and distributions centered around a non-zero value. Distributions centered around a non-zero value allow to model the case in which the modal signal of one variable about another is informative. This is in contrast to scenarios in which the modal signal is uninformative. We consider both scenarios as natural antithetical cases to study. We re-center the Beta Distributions around zero by simply subtracting the mean of the original distribution from each draw.    

Additionally, we use the Student's t-Distribution and the Lognormal distribution to assess the robustness of our results to different distributional assumptions. The Student's t-Distribution presents the particular advantage that its parametrization allows to directly control the tail-behavior of the distribution. We consider fat tails to be a relevant scenario as it allows to model the case in which most variables are uninformative about each other, except for outliers with very high correlation coefficients. This captures the case in which learning is essentially flat until there is a ``lucky draw'' which substantially increases prediction accuracy. We think of fat tail distributions as modeling the scenario of ``edge case predictions'' in which a firm aims to predict an idiosyncratic variable for which most other variables have little value, except for some rare exceptions.   

%We simulate the signal strength between any random pair of variables by assuming different distributions for the correlation coefficients. Our simulation approach allows us to study a range of scenarios. In one case, variables may, on average, convey strong signals about one another. In another case, variables may typically convey very weak signals about one another, with (very) rare exceptions of a strong signal between a random pair.

\subsubsection*{Overfitting}

In our model, additional variables will always weakly increase the prediction accuracy. In real-world applications, adding ``too much'' variables may lead to a worse out-of-sample prediction accuracy. This phenomenon, known as overfitting, may lead a firm to discard additional variables. The overfitting problem is a result of the finiteness of the training data, which leads a model to pick up erroneous patterns that are not present in the real data. With infinite training data, every variable that leads to a marginal increase in prediction accuracy will be accurately estimated and therefore also lead to an increase of out-of-sample performance. Our setting, which implicitly assumes infinite training data, can therefore be thought to abstract away from the overfitting problem. 

However, an alternative interpretation of our setting is that it only accounts for the variables which actually prove to increase out-of-sample performance, and implicitly discards those that do not. This is consistent with the notion that a firm will only add a variable to its model if it increases out-of-sample performance. Additionally, a variable that first appears not useful might prove valuable later on as more new variables accumulate, which may lead the firm to use a new model which includes variable previously not used. Therefore, our implicit assumption that a new will never decrease the prediction accuracy seem aligned with the behavior of a firm that only deploys models after testing their out-of-sample performance.  




